Let there be a clock on the beach: Reducing Object Hallucination in Image Captioning

Explaining an image with missing or non-existent objects is known as object bias (hallucination) in image captioning. This behaviour is quite common in the state-of-the-art captioning models which is not desirable by humans. To decrease the object hallucination in captioning, we propose three simple yet efficient training augmentation method for sentences which requires no new training data or increase in the model size. By extensive analysis, we show that the proposed methods can significantly diminish our models' object bias on hallucination metrics. Moreover, we experimentally demonstrate that our methods decrease the dependency on the visual features. All of our code, configuration files and model weights will be made public.

==> related.tex <==
\section{Related Work}
Following the advances of the encoder-decoder framework~\cite{Cho2014} with attention~\cite{Bahdanau2014} in machine translation, automatic image captioning took off using similar architectures~\cite{vinyals2015show, Xu2015}. The next advance in captioning came from using a pretrained object detector as feature extractor with two types of attention, top-down and bottom-up attention~\cite{anderson2017bottom}. In parallel, it was demonstrated that training captioning models with the REINFORCE algorithm~\cite{williams1992simple}, optimizing the evaluation metrics directly, had benefits over using cross-entropy loss~\cite{rennie2017self}. More recently, with the presentation of Transformers~\cite{vaswani2017attention}, a new family of models~\cite{huang2019attention} achieved state-of-the-art results. 

Nevertheless, despite the continuous improvement on the classic captioning metrics, there are many biases exploited, that produce biases in the models. To compensate for gender bias where the models are known to prefer a certain gender over the other in specific settings,~\cite{hendricks2018women} proposed to tweak the original cross-entropy loss with confidence/appearance loss. On confidence loss, they employ binary cross-entropy loss to predict the word woman higher than man if the picture includes woman. On the confusion loss, they occlude the images containing person with segmentation map and they propose to discard the prediction of the gender word.  

Another bias in captioning is related to action bias where certain actions are preferred over others described by~\cite{yang2020deconfounded} where they employ causality~\cite{pearl2009causality} into the captioning models. More specifically, their proposed method uses 4 layers LSTM with running expected average on ConceptNet~\cite{liu2004conceptnet} concepts for each word produced in the caption, which it introduces a significant computation overload.

In addition,~\cite{rohrbach2018object} showed that contemporary captioning models are prone to object bias. Moreover, they describe that evaluation metrics merely measure the similarity between the ground truth and produced caption, not capturing image relevance. Consequently, they propose two metrics to  quantify the degree of hallucination of objects, namely CHAIRs and CHAIRi. CHAIR metrics evaluates how much our models produced wrong object labels at sentence level (hence CHAIRs) and at object level (hence CHAIRi). 

Surprisingly, the object hallucination problem has not received the attention it deserves. 
% , especially given the fact that image captioning is driven from an application point of view. 
In this work, we try to diminish object bias without enlarging the model size or using extra data. We do so following a simple strategy that can be used with any model that accepts object detection features as inputs.
% We hope to provoke the community to work on ``simple'' ideas to reduce object bias.
